Memory Wrap: a Data-Efficient and Interpretable Extension to Image Classification Models

Due to their black-box and data-hungry nature, deep learning techniques are not yet widely adopted for real-world applications in critical domains, like healthcare and justice. This paper presents Memory Wrap, a plug-and-play extension to any image classification model. Memory Wrap improves both data-efficiency and model interpretability, adopting a content-attention mechanism between the input and some memories of past training samples. We show that Memory Wrap outperforms standard classifiers when it learns from a limited set of data, and it reaches comparable performance when it learns from the full dataset. We discuss how its structure and content-attention mechanisms make predictions interpretable, compared to standard classifiers. To this end, we both show a method to build explanations by examples and counterfactuals, based on the memory content, and how to exploit them to get insights about its decision process. We test our approach on image classification tasks using several architectures on three different datasets, namely CIFAR10, SVHN, and CINIC10.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \answerYes{}
  \item Did you describe the limitations of your work?
  \answerYes{\bf{See Sect.~\ref{sec:discussion} and App.~\ref{appx:cost}}}
  \item Did you discuss any potential negative societal impacts of your work?
  \answerYes{\bf{We added a brief discussion about a potential amplification of bias, how to identify it (Sect. \ref{sec:results-explanations}) and possible solutions in Sect.~\ref{sec:discussion}}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
  \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  \answerYes{\bf{see README}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  \answerYes{\bf{See App.~\ref{appx:trainingdetails} and Sect.~\ref{sec:results-setup}}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{\bf{We ran each experiment 15 times reporting the error margin.}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{\bf{See App.~\ref{appx:trainingdetails} for type of resources and 1.5 for computational cost.}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  \answerYes{}
  \item Did you mention the license of the assets?
  \answerYes{\bf{See App.~\ref{appx:trainingdetails}}}
  \item Did you include any new assets either in the supplemental material or as a URL?
  \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/majorvoting.tex <==
\subsection{Major Voting Baseline}
\label{appx:majorvoting}
As an additional baseline we consider the predictions obtained applying a major voting algorithm on the content of the memory set.

Let be: $M_{ec} = \{f(x^m_j)\}$ the set of encodings
of memory samples associated with a weight $w_j > 0$; $Y_{ec} $ the set of targets associated to the samples; and $\hat{Y}_{ec} = g(x^m_j)$ the predictions obtained using the memory set as the input of the network.
The major voting algorithm will choose as class of the given input the most common prediction in $Y_{ec}$ or in $\hat{Y}_{ec}$. We observed that the accuracies of both method are the sames, the only change is that the first requires to know a priori the targets of the samples in the memory set, while the second is slower due to the time required to obtain the additional predictions. Therefore for simplicity we report only one result valid for both of them.
\begin{table*}[h!]
  %\setlength{\tabcolsep}{4pt}
    \centering
    \caption{Avg. accuracy and standard deviation comparison on SVHN
    dataset between the standard model and the variants of Memory Wrap. The
    comparison highlights the difference in performance when using a subset of
    the dataset in the range \{1k,2k,5k\} as training set. The accuracy is
    computed as the mean over 15 runs. For each configuration, we highlight in bold the best result and results that are within its margin.}
    \label{table:mvSVHN}
    \begin{tabular}[t]{@{}rrrrrr@{}}
      \toprule
      \multicolumn{5}{c}{\textbf{SVHN Avg. Accuracy\%}}\\
      \midrule
       &&\multicolumn{3}{c}{\textbf{Samples}}\\
       Model&Variant&1000&2000&5000\\
      \midrule
      \quad EfficientNetB0 &Only Memory    &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \quad &Major Voting      &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \quad &Memory Wrap   &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \quad &Major Voting     &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \midrule
      \quad MobileNet&Only Memory     &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \quad &Major Voting     &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \quad &Memory Wrap      &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \quad &Major Voting      &  $\pm$   &  $\pm$   &  $\pm$  &\\
      \midrule
      \quad ResNet18 &Only Memory   & 37.57 $\pm$ 6.48 & 68.87 $\pm$ 8.73   &  87.62 $\pm$ 0.44 \\
      \quad &Major Voting     & 36.62 $\pm$ 5.89 &  62.26 $\pm$ 8.41 & 83.99 $\pm$ 0.71 \\
      \quad &Memory Wrap    & 45.30 $\pm$ 8.20  &  $\pm$ &  $\pm$\\
      \quad &Major Voting   & 41.71 $\pm$  6.65 & $\pm$  &  $\pm$  \\
      \bottomrule
    \end{tabular}
  
  \end{table*}

  \begin{table*}[h!]
    %\setlength{\tabcolsep}{4pt}
      \centering
      \caption{Avg. accuracy and standard deviation comparison on CIFAR10
      dataset between the variant of Memory Wrap that uses only the memory and the major voting baseline. The
      comparison highlights the difference in performance when using a subset of
      the dataset in the range \{1k,2k,5k\} as training set. The accuracy is
      computed as the mean over 15 runs. For each configuration, we highlight in bold the best result and results that are within its margin.}
      \label{table:mvCIFAR10}
      \begin{tabular}[t]{@{}rrrrrr@{}}
        \toprule
        \multicolumn{5}{c}{\textbf{CIFAR10 Avg. Accuracy\%}}\\
        \midrule
         &&\multicolumn{3}{c}{\textbf{Samples}}\\
         Model&Variant&1000&2000&5000\\
        \midrule
        \quad EfficientNetB0 &Only Memory     & \textbf{40.64 $\pm$  2.05} & \textbf{52.87 $\pm$ 2.09}  & \textbf{70.83 $\pm$ 0.56} \\
        \quad &Major Voting      & 40.35 $\pm$ 2.02  &  52.46 $\pm$ 2.09  & 70.38 $\pm$ 0.57 \\
        \quad &Memory Wrap    & \textbf{41.45 $\pm$ 0.76}  & \textbf{52.83 $\pm$ 1.38}  & \textbf{70.48 $\pm$ 0.78}\\
        \quad &Major Voting     &  41.04 $\pm$ 0.75   &  52.24 $\pm$ 1.44  & 69.41 $\pm$ 0.79 \\
        \midrule
        \quad MobileNet&Only Memory     &  $\pm$   &  $\pm$   &  $\pm$  &\\
        \quad &Major Voting     &  $\pm$   &  $\pm$   &  $\pm$  &\\
        \quad &Memory Wrap      &  $\pm$   &  $\pm$   &  $\pm$  &\\
        \quad &Major Voting      &  $\pm$   &  $\pm$   &  $\pm$  &\\
        \midrule
        \quad ResNet18 &Only Memory     & \textbf{40.34 $\pm$ 0.90}  & \textbf{51.14 $\pm$ 1.21}  &   \textbf{70.25  $\pm$ 0.78}  \\
        \quad &Major Voting   & 39.35 $\pm$  0.81 & 50.29 $\pm$  1.20 &   69.41 $\pm$ 0.72 \\
        \quad &Memory Wrap    & \textbf{40.90 $\pm$ 1.27}  &  \textbf{51.14 $\pm$ 1.16}  &  \textbf{69.86 $\pm$ 0.72} \\
        \quad &Major Voting   & 39.71 $\pm$ 1.12  & 50.09 $\pm$  1.12 &   68.98 $\pm$ 0.67 \\
        \bottomrule
      \end{tabular}
    
    \end{table*}
